Dynamic Reserve Prices for Repeated Auctions: Learning from Bids

A large fraction of online advertisement is sold via repeated second price auctions. In these auctions, the reserve price is the main tool for the auctioneer to boost revenues. In this work, we investigate the following question: Can changing the reserve prices based on the previous bids improve the revenue of the auction, taking into account the long-term incentives and strategic behavior of the bidders? We show that if the distribution of the valuations is known and satisfies the standard regularity assumptions, then the optimal mechanism has a constant reserve. However, when there is uncertainty in the distribution of the valuations, previous bids can be used to learn the distribution of the valuations and to update the reserve price. We present a simple, approximately incentive-compatible, and asymptotically optimal dynamic reserve mechanism that can significantly improve the revenue over the best static reserve. The paper is from July 2014 (our submission to WINE 2014), posted later here on the arxiv to complement the 1-page abstract in the WINE 2014 proceedings.

==> 5_transient_valuations.tex <==
\subsection{Transient Valuations} \label{sec:transient}
%
So far we assumed that the valuations of the agents are constant over time. In this section, we consider the following extension of our model: each time an agent participates, he draws a new valuation from $F_s$ independently with some probability $\beta$ (our original model  corresponds to the case $\beta =0$), and retains his previous valuation with probability $1-\beta$.

We observe that our incentive compatibility results hold in this setting because the incentive of the agents for deviation is even smaller and the proofs of Theorem \ref{thm:approx_Nash} and \ref{thm:approx_BNE} work nearly as before for any $\beta \in [0,1]$. % (with some additional slack).
In addition, Theorem~\ref{thm:no_improve_n_equal_1} holds if we consider mechanisms that are periodic ex-post individually rational~\citep{BergemannV10}; in other words, the utility of any truthful agent at the end of each round $t$, $1\le t\le T$ should be non-negative.

The following example shows that a mechanism that is not ex-post individually rational can obtain a higher revenue by charging the agents a high price in advance: Suppose there is only one agent ($n=1$), the agent participates in all rounds ($\alpha=1$),  and the agent draws a new valuation at each round from the uniform distribution over $[0,1]$ ($\beta=1$). It is not difficult to see that the optimal constant reserve for this setting is equal to ${1\over 2}$ which yields the expected revenue of ${T\over 4}$ since the agent will purchase the item with probability ${1\over 2}$. Now consider a mechanism that offers reserve price ${T-1\over 2}-\varepsilon$ (for an arbitrarily small $\varepsilon$) in the first round and if the agent accepts that price, the mechanism offers the item for free in the future rounds and if the agent refuses the offer will post the price of $1$ at each round. Observe that the agent will accept the mechanism's offer in the first round and the revenue obtained in this case is equal to ${T-1\over 2}-\varepsilon$. However, this mechanism is not ex-post individually rational. For $\beta\in(0,1)$ the optimal mechanism (that does not satisfy the ex-post IR property) would take the form of contracts followed by sequence of auctions~\citep{KakadeLN13,Battaglini05}.

==> two_periods.tex <==
\section{Short Horizon: $T=2$}
%
In this section, we consider an important special case of our model where the length of the horizon is equal to $T=2$.
In this case, for all agents, the weakly dominant strategy of each agent in the second round is to be truthful. This allows us to focus on the bidding strategy of the agents only in the first period. cite athey

%

\subsection{Examples}

We can construct an example where the dynamic reserve leads to a benefit as follows:
Consider a distribution on $s \in \{ L, H \}$, and $F_L$ and $F_H$ with unbounded supports such that the unique optimal static reserve (assuming just one bidder, if that matters) is $r_1$ close to $r_L$. Suppose that bidder 2 is always present, i.e.,  $\alpha_2=1$. Now suppose bidder 1 appears in each round independently with a small probability $\alpha_1$. For $\alpha_1$ small enough, the optimal static reserve is still $r_1$. Consider the mechanism $M(r_1, \rho, i, r_1, r_H)$:
\begin{itemize}
  \item For bidder 2, the threshold $\theta_{H,2} \xrightarrow{\alpha_1 \rightarrow 0} \infty$ and $\theta_{L,2}$ is even larger, i.e., bidder 2 almost always shades if $v_2>\rho$, because he thinks it is unlikely that bidder 1 will show up.
  \item For bidder 1, the threshold $\theta_{H,1} \xrightarrow{\alpha_1 \rightarrow 0} \rho$ and $\theta_{L,1} \xrightarrow{\alpha_1 \rightarrow 0} \rho$ as well, i.e., bidder 1 almost always tells the truth, because he thinks it is unlikely he will come back in round 2.
  \item In cases where bidder 1 does not show up in the first round, the allocation and revenue of this mechanism is identical to the mechanism with static reserve $r_1$. However in cases when bidder 1 does show up in round $1$ and $s=H$, there are two competing effects:
      \begin{itemize}
        \item Loss in round 1 revenue due to shading by bidder 2.
        \item Gain in round 2 revenue due to raising the reserve to $H$.
      \end{itemize}
      The second effect should be greater for a wide range of distributions $p_s, F_L, F_H$. There is a much smaller effect of the case when bidder 1 has $v_1>\rho$ for $s=L$, which causes very limited loss.
\end{itemize}


%DO NOT ERASE
%\begin{proof}
%%
%Let $v_1 = v$.
%It is easy to see that for $v\le\rho$,  being truthful is a (weakly) dominant strategy.
%
%Define shading strategy as bidding equal to $\rho$ for $v>\rho$.
%Since $v\ge\rho \ge r_H$, we have
%
%\begin{eqnarray*}
%\utruth & = & \alpha_2 \left(\max\{F_s(v)-F_s(\thetab),0\} v - \int_{\thetab}^{\max\{\thetab,v\}} x f(x) dx \right) \\
%& & + \alpha_2 \left((F_s(\thetab)-F_s(\rho))(v-\rho) + F(\rho) v - \left(\int_{r_L}^{\rho} x f_s(x) dx  + F_s(r_L) r_L \right)\right) \\
%& & + \alpha_2 (\alpha_1 \alpha_2) \left(F_s(v) v - \left(\int_{r_H}^{v} x f_s(x) dx + F_s(r_H) r_H\right)\right) \\
%& & + \alpha_2 (\alpha_1 (1-\alpha_2)) (v-r_H) \\
%& & + (1-\alpha_2) \left(v-r_L\right) \\
%& & + (1-\alpha_2) \alpha_1 \left(\alpha_2 \left(F_s(v) v - \left(\int_{r_H}^{v} x f_s(x) dx + F_s(r_H) r_H\right)\right) + (1-\alpha_2) (v-r_H)\right)
%\end{eqnarray*}
%
%
%\begin{eqnarray*}
%\ushade & = & \alpha_2 \left((F_s(\thetab)-F_s(\rho)){v-\rho\over 2} + F(\rho) v - \left(\int_{r_L}^{\rho} x f_s(x) dx  + F_s(r_L) r_L \right)\right) \\
%& & + \alpha_2 (\alpha_1 \alpha_2) \left(F_s(v) v - \left(\int_{r_L}^{v} x f_s(x) dx + F_s(r_L) r_L \right)\right) \\
%& & + \alpha_2 (\alpha_1 (1-\alpha_2)) (v- (F_s(\thetab) r_L + (1-F_s(\thetab)) r_H)) \\
%& & + (1-\alpha_2) \left(v-r_L\right) \\
%& & + (1-\alpha_2) \alpha_1 \left(\alpha_2 \left(F_s(v)v - \left(\int_{r_L}^{v} x f_s(x) dx + F_s(r_L) r_L\right)\right) + (1-\alpha_2) (v-r_L)\right)
%\end{eqnarray*}
%
%\begin{eqnarray*}
%& & \utruth - \ushade \\
%& = &  \alpha_2 \left(\max\{F_s(v)-F_s(\thetab),0\} v - \int_{\thetab}^{\max\{\thetab,v\}} x f(x) dx \right) \\
%& & + \alpha_2 (F_s(\thetab)-F_s(\rho)){v-\rho\over 2} \\
%& & + \alpha_2 (\alpha_1 \alpha_2)  \left(\int_{r_L}^{r_H} x f_s(x) dx + F_s(r_L) r_L - F_s(r_H) r_H \right) \\
%& & - \alpha_2 (\alpha_1 (1-\alpha_2)) (F_s(\thetab)) r_H - (F_s(\thetab) r_L) \\
%& & + (1-\alpha_2) \alpha_1 \left(\alpha_2 \left(\int_{r_L}^{r_H} x f_s(x) dx  + F_s(r_L) r_L - F_s(r_H) r_H \right) + (1-\alpha_2) (r_L-r_H)  \right) \\
%& = & \alpha_2 \left(\max\{F_s(v)-F_s(\thetab),0\} v - \int_{\thetab}^{\max\{\thetab,v\}} x f(x) dx + (F_s(\thetab)-F_s(\rho)){v-\rho\over 2} \right) \\
%& &  + \alpha_1 \alpha_2  \left(\int_{r_L}^{r_H} x  f_s(x) dx + F_s(r_L)r_L - F_s(r_H) r_H \right) \\
%& & - \alpha_2 (\alpha_1 (1-\alpha_2)) (F_s(\thetab)) r_H - (F_s(\thetab) r_L) \\
%& & - (1-\alpha_2) \alpha_1 (1-\alpha_2) (r_H-r_L)
%%\\
%\end{eqnarray*}
%
%Observe that $\utruth - \ushade$ is increasing in $v$. Therefore, there exists a threshold $\thetap$ such that threshold strategy $(\rho,\thetap)$ is a best response for the first bidder.
%
%%DO NOT ERASE
%%\item $v\in[\rho,\thetab]$ and $v<r_H$:
%%
%%\begin{eqnarray*}
%%\ushade & = & \alpha_2 \left((F_s(\thetab)-F_s(\rho)){v-\rho\over 2} + F(\rho) v - \left(\int_{r_L}^{\rho} x f_s(x) dx  + F_s(r_L) r_L\right) \right) \\
%%& & + \alpha_2 \alpha_1 \left(\alpha_2 \left(F_s(v) v - \left(\int_{r_L}^{v} x f_s(x) dx + F_s(r_L) r_L\right)\right) + (1-\alpha_2) F_s(\thetab) (v-r_L)\right) \\
%%& & + (1-\alpha_2) \left(v-r_L\right) \\
%%& & + (1-\alpha_2) \alpha_1 \left(\alpha_2 \left( F_s(v) v - \left(\int_{r_L}^{v} x f_s(x) dx + F_s(r_L) r_L\right)\right) + (1-\alpha_2) (v-r_L)\right)
%%\end{eqnarray*}
%%
%%\begin{eqnarray*}
%%\utruth & = & \alpha_2 \left((F_s(\theta_H)-F_s(\rho))(v-\rho) + \left(F(\rho)\rho - \left(\int_{r_L}^{\rho} x f_s(x) dx  + F_s(r_L) r_L \right)\right)\right) \\
%%& & + (1-\alpha_2) \left(v-r_L\right)
%%\end{eqnarray*}
%%
%%\begin{eqnarray*}
%% \ushade - \utruth & = & - \alpha_2 \left((F_s(\thetab)-F_s(\rho)){v-\rho\over 2}\right) \\
%%& & + \alpha_2 \alpha_1 \left(F_s(v) v - \left(\int_{r_L}^{v} x f_s(x) dx + F_s(r_L) r_L\right)\right) \\
%%& & + \alpha_2 \alpha_1 (1-\alpha_2) \left(F_s(\thetab) (v-r_L)\right) \\
%%& & + (1-\alpha_2) \alpha_1 \left((1-\alpha_2) (v-r_L)\right) \\
%%& = & - \alpha_2 \left((F_s(\thetab)-F_s(\rho)){v-\rho\over 2}\right) \\
%%& & + \alpha_2 \alpha_1 \left(\int_{r_L}^{v} F_s(x) dx \right) \\
%%& & + \alpha_1 (1-\alpha_2) \left(\alpha_2  F_s(\thetab) + (1-\alpha_2)\right) (v-r_L)
%%\end{eqnarray*}
%%
%%\begin{eqnarray*}
%%{\partial \left(\ushade - \utruth \right) \over \partial v} & = & -  (F_s(\thetab)-F_s(\rho)){\alpha_2\over 2} \\
%%& & + \alpha_2 \alpha_1  F_s(v) \\
%%& & + (1-\alpha_2) \alpha_1 \Bigl((1-\alpha_2(1-F_s(\thetab))\Bigr) \\
%%\end{eqnarray*}
%
%\end{proof}

